Private Continual Release of Real-Valued Data Streams

We present a differentially private mechanism to display statistics (e.g., the moving average) of a stream of real valued observations where the bound on each observation is either too conservative or unknown in advance. This is particularly relevant to scenarios of real-time data monitoring and reporting, e.g., energy data through smart meters. Our focus is on real-world data streams whose distribution is light-tailed, meaning that the tail approaches zero at least as fast as the exponential distribution. For such data streams, individual observations are expected to be concentrated below an unknown threshold. Estimating this threshold from the data can potentially violate privacy as it would reveal particular events tied to individuals [1]. On the other hand an overly conservative threshold may impact accuracy by adding more noise than necessary. We construct a utility optimizing differentially private mechanism to release this threshold based on the input stream. Our main advantage over the state-of-the-art algorithms is that the resulting noise added to each observation of the stream is scaled to the threshold instead of a possibly much larger bound; resulting in considerable gain in utility when the difference is significant. Using two real-world datasets, we demonstrate that our mechanism, on average, improves the utility by a factor of 3.5 on the first dataset, and 9 on the other. While our main focus is on continual release of statistics, our mechanism for releasing the threshold can be used in various other applications where a (privacy-preserving) measure of the scale of the input distribution is required.

==> related.tex <==
\section{Related work}
As mentioned before, the privacy-preserving algorithms for continual release of statistics from binary streams described in~\cite{cont-release, cont-observe} can be modified to the scenario addressed in this paper, i.e., release of statistics from a sequence whose values are from the real interval $[0, B]$. Indeed, we have used the algorithm from~\cite{cont-release} as one of the components of our method. However, the focus of the two works in~\cite{cont-release} and {cont-observe} is on improving the error for binary strings which do not have the added factor of $B$. 

The two aforementioned algorithms are based on event-level privacy. As such, if the aim of privacy is to protect all events from an individual (e.g., all trips made by an individual over the course of the whole year), then the privacy provided by these algorithms is insufficient. The work from~\cite{w-event} attempts to improve this by offering privacy for up to $w$ successive events. Noting that any $w$ successive events might not contain multiple events originating from a single individual, the authors from~\cite{} introduce $l$-trajectory privacy, where any successive $l$ events from a user is targeted for privacy~\cite{l-trajectory}. Note that these variations of the definition of differential privacy rely on how a neighbouring stream is defined. We note that our method can be easily used in conjunction with algorithms for these variants of privacy, as we only use the algorithm from~\cite{cont-release} as a submodule. However, to work out a suitable threshold in a differentially private manner for any variant in the definition of neighbouring streams requires tweaking our algorithm. This is an interesting area of work for future research.     

%This contunal counting issue as already been tackled in \cite{cont-release}, \cite{cont-observe},  but in theses case, streams were determistist binary streams. And, in our case we based our work on the algorithm develloped in \cite{cont-release} : the binary algorithm for counting limited streams. The main idea behind this work is to arrange the sums in a way that leaks less information. Because of this we can reduce the scale of the laplacian noise, and then increase the accuracy of the sum.

Our work on estimating the threshold using the $p$-quantile can be thought as an exercise in finding robust statistics with differential privacy; a line of work that was discussed in~\cite{robust-stats}.
%Robusts statistics in order to make statistic inferences is also on other major aspect of this paper, and it was also develloped in \cite{robust-stats}. 
Our approach was to use smooth sensitivity to obtain the threshold. \textcolor{red}{The reason for this was that it was simpler to use it with an optimization algorithm.} 
Instead, we could also try and adapt the algorithms developed in \cite{robust-stats}, and improve them using smooth sensitivity as is done in our technique for estimating the $p$-quantile. 
%for instance if we have a single value that is very far away, smooth sensitivity could be too big).}
